Angular velocity of gravitational radiation from precessing binaries and the corotating frame

This paper defines an angular velocity for time-dependent functions on the sphere, and applies it to gravitational waveforms from compact binaries. Because it is geometrically meaningful and has a clear physical motivation, the angular velocity is uniquely useful in helping to solve an important---and largely ignored---problem in models of compact binaries: the inverse problem of deducing the physical parameters of a system from the gravitational waves alone. It is also used to define the corotating frame of the waveform. When decomposed in this frame, the waveform has no rotational dynamics and is therefore as slowly evolving as possible. The resulting simplifications lead to straightforward methods for accurately comparing waveforms and constructing hybrids. As formulated in this paper, the methods can be applied robustly to both precessing and nonprecessing waveforms, providing a clear, comprehensive, and consistent framework for waveform analysis. Explicit implementations of all these methods are provided in accompanying computer code.

==> 3DPreamble.tex <==
%auto-ignore

%% This file contains preamble stuff needed to embed 3D asymptote PDFs
%% directly into a paper.  It is not needed if there are no such PDFs.

\usepackage[bigfiles]{media9}

\def\ASYprefix{}
\newbox\ASYbox
\newdimen\ASYdimen
\long\def\ASYbase#1#2{\leavevmode\setbox\ASYbox=\hbox{#1}\ASYdimen=\ht\ASYbox%
\setbox\ASYbox=\hbox{#2}\lower\ASYdimen\box\ASYbox}
\long\def\ASYaligned(#1,#2)(#3,#4)#5#6#7{\leavevmode%
\setbox\ASYbox=\hbox{#7}%
\setbox\ASYbox\hbox{\ASYdimen=\ht\ASYbox%
\advance\ASYdimen by\dp\ASYbox\kern#3\wd\ASYbox\raise#4\ASYdimen\box\ASYbox}%
\put(#1,#2){#5\wd\ASYbox 0pt\dp\ASYbox 0pt\ht\ASYbox 0pt\box\ASYbox#6}}%
\long\def\ASYalignT(#1,#2)(#3,#4)#5#6{%
\ASYaligned(#1,#2)(#3,#4){%
\special{pdf:q #5 0 0 cm}%
}{%
\special{pdf:Q}%
}{#6}}
\long\def\ASYalign(#1,#2)(#3,#4)#5{\ASYaligned(#1,#2)(#3,#4){}{}{#5}}
\def\ASYraw#1{#1}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

